Quantum Repeater using Two-Mode Squeezed States and Atomic Noiseless Amplifiers

We perform a theoretical investigation into how a two-mode squeezed vacuum state, that has undergone photon loss, can be stored and purified using noiseless amplification with a collection of solid-state qubits. The proposed method may be used to probabilistically increase the entanglement between the two parties sharing the state. The proposed amplification step is similar in structure to a set of quantum scissors. However, in this work the amplification step is realized by a state transfer from an optical mode to a set of solid-state qubits, which act as a quantum memory. We explore two different applications, the generation of entangled many-qubit registers, and the construction of quantum repeaters for long-distance quantum key distribution.

==> Text/Registers.tex <==
\subsection{Generating Entangled Registers}
We initialize the optical channel into an entangled state:
\begin{equation}
	\ket{\psi} = \sum_{n=0}^{\infty} c_n \ket{n}_L\ket{n}_R
\end{equation}
The subscript $L$ and $R$ indicates whether we are referring to the left part of the state or the right part.
We let the optical mode be a two-mode squeezed vacuum state, with the coefficients:
\begin{equation}
	c_n = (-e^{i \phi})^n  \sqrt{\frac{\langle n \rangle^n}{(1+\langle n \rangle )^{n+1}}}
\end{equation}
Where $\langle n \rangle$ is the average number of photons in the TMSV. In this work we consider the case where the phase $\phi$ is set to 0. Focusing on the left side of Figure \ref{Analysis:Figure:Layout}. We split up the optical mode on $N$ beamsplitters. We intend to split the optical field evenly among the $N$ modes, to do this we use the transmission and reflection coefficients:
\begin{align}
	t_j = \sqrt{\frac{j-1}{j}}, \hspace{1cm} 	r_j = \sqrt{\frac{1}{j}}
\end{align}
Where $j$ is the number of the arm, starting from 1 at the leftmost arm.
As a result, the amplitude operator for the left part of the TMSV, $a_L$, splits into the $N$ arms as:
\begin{equation}
	a_L \rightarrow \sqrt{\frac{1}{N}} \sum_{k=1}^{N} a_k
\end{equation}
$\ket{\psi}$ then transforms as:
\begin{align}
	\ket{\psi} & = \sum_{n=0}^{\infty} c_n \frac{(a_L^\dagger)^n}{\sqrt{n!}}\ket{0}_L\ket{n}_R\\ &\rightarrow \sum_{n=0}^{\infty} c_n \frac{1}{\sqrt{n!}} \left( \sqrt{\frac{1}{N}} \right)^n (a_1^\dagger + a_2^\dagger + \cdots + a_N^\dagger)^n \ket{0}_l\ket{n}_R
\end{align}
Note that we also propagated $\ket{0}_L$ to $\ket{0}_l$ with the latter being the empty $l$ modes at the left register. Using the multinomial theorem, we may rewrite the ladder operator product as:
\begin{align}
	&(a_1^\dagger + a_2^\dagger + \cdots + a_N^\dagger)^n \ket{0}_l \\ &= \sum_{j_1 + j_2 + \cdots + j_N = n} \frac{n!}{j_1! j_2! \cdots j_N!} \left(a_1^{\dagger}\right)^{j_1} \left(a_2^{\dagger}\right)^{j_2} \cdots \left(a_N^{\dagger}\right)^{j_N} \ket{0}_l \\ &= \sum_{j_1 + j_2 + \cdots + j_N = n} \frac{n!}{j_1! j_2! \cdots j_N!} \sqrt{j_1!}\sqrt{j_2!} \cdots \sqrt{j_N!} \ket{j_1,j_2,\cdots,j_N}_l\\ & = \sum_{\mathbf{j}_n} \Omega_{\mathbf{j}_n} \ket{\mathbf{j}_n}_l
\end{align}
Where the final sum $ \sum_{\mathbf{j}_n}$ runs over unique strings $\mathbf{j}_n = (j_1,j_2,\cdots,j_N)$ such that $j_1+j_2+\cdots+j_N = n$. $\Omega_{\mathbf{j}_n}$ is the prefactor given by:
\begin{align}
    \Omega_{\mathbf{j}_n} = \frac{n!}{\sqrt{j_1!}\sqrt{j_2!} \cdots \sqrt{j_N!}}
\end{align}
Using this notation we then write $\ket{\psi}$ as:
\begin{align}
	\ket{\psi} & =  \sum_{n=0}^{\infty} c_n \frac{1}{\sqrt{n!}} \left( \sqrt{\frac{1}{N}} \right)^n \sum_{\mathbf{j}_n} \Omega_{\mathbf{j}_n} \ket{\mathbf{j}_n}_l \ket{n}_R
	\label{NoErrors:Equation:psi1}
\end{align}
Meanwhile, we initialize the left registry in the state:
\begin{equation}
	\ket{L} = \prod_{k=1}^{N} (\cos(\theta_L)\ket{0}_{q_k} \ket{0}_{f_k} + \sin(\theta_L)\ket{1}_{q_k} \ket{1}_{f_k})
	\label{NoErrors:Equation:L}
\end{equation}
Where the notation $\ket{0}_{q_k} \ket{0}_{f_k}$ indicates that for arm $k$, the qubit ($q_k$) is in the state 0 and the fiber ($f_k$) coupled to the qubit is occupied by 0 photons.\\
We may then write $\ket{L}$ as:
\begin{align}
	\ket{L} &= \sum_{a_1=\{0,1\}} \sum_{a_2=\{0,1\}} \cdots \sum_{a_N=\{0,1\}} \nonumber \\
	& \cos(\theta_L)^{(1-a_1)} \sin(\theta_L)^{a_1} \cdots \cos(\theta_L)^{(1-a_N)} \sin(\theta_L)^{a_N} \ket{a_1}_{q_1}\ket{a_1}_{f_1}\cdots \ket{a_N}_{q_N}\ket{a_N}_{f_N} \nonumber \\
	& = \sum_{\mathbf{a}} \beta(\mathbf{a},\theta_L) \ket{\mathbf{a}}_q \ket{\mathbf{a}}_f
	\label{NoErrors:Equation:Register}
\end{align}
Where we've  introduced a sum over binary lists $\sum_{\mathbf{a}}$ leaving the registry in a superposition of binary states $\ket{\mathbf{a}}_q \ket{\mathbf{a}}_f = \ket{a_1}_{q_1}\ket{a_1}_{f_1}\cdots \ket{a_N}_{q_N}\ket{a_N}_{f_N}$. We've also introduced the parameter $\beta(\mathbf{a},\theta_L)$ to take the angle $\theta_L$ into account. 
We interact $\ket{\psi}$ and $\ket{L}$ using $N$ beamsplitters and measure on the modes using the photon resolving detectors $T$ and $B$ for each arm. We assume a particular measurement outcome $(t_k,b_k)_k$, indicating that $t_k$ photons are going to detector $T_k$ and $b_k$ photons are going to detector $B_k$ in arm $k$. Subject to this measurement, the state transforms as:
\begin{align}
	\ket{\psi} \ket{L} \rightarrow \bra{t_1}_{T_1}\bra{b_1}_{B_1} U_1 \bra{t_2}_{T_2}\bra{b_2}_{B_2} U_2 \cdots \bra{t_N}_{T_N}\bra{b_N}_{B_N} U_N \ket{\psi} \ket{L} 
	\label{NoErrors:Equation:ParticularMeasurement}
\end{align}
Where $U_k$ is the beamsplitter in arm $k$. The bra acting from the left then indicates the projective action of the photon resolving detectors. \\
The right part of the TMSV state is entangled with the left registry qubit $k$ if $t_k + b_k = 1$ since the photon could then have come from either the TMSV state or the bright state of the qubit. Other measurement outcomes tend to yield information about the state of the registry and the TMSV state and are expected to lower the entanglement, though this assumption could be explored further. In this work we will only accept measurement outcomes where $t_k + b_k = 1$ for all $N$ arms of the registers. \\
To evaluate the above expression, we let the beamsplitters act on the bra. Eg. we examine:
\begin{equation}
	\bra{t_k}_{T_k}\bra{b_k}_{B_k} U_k = (U_k^\dagger \ket{t_k}_{T_k}\ket{b_k}_{B_k})^\dagger
\end{equation}
First let $t_k = 1$ and $b_k = 0$, we assume balanced beamsplitters:
\begin{equation}
	U_k^\dagger \ket{1}_{T_k}\ket{0}_{B_k} = \frac{1}{\sqrt{2}} \left( \ket{0}_{f_k} \ket{1}_{l_k} + \ket{1}_{f_k} \ket{0}_{l_k} \right)
\end{equation}
When we let $t_k = 0$ and $b_k = 1$, we get:
\begin{equation}
	U_k^\dagger \ket{0}_{T_k}\ket{1}_{B_k} = \frac{1}{\sqrt{2}} \left( \ket{0}_{f_k} \ket{1}_{l_k} - \ket{1}_{f_k} \ket{0}_{l_k} \right)
\end{equation}
As required by the reciprocity relations. Evidently, measuring  $t_k = 0$ and $b_k = 1$ phase shifts registry qubit $k$ by $\pi$ if it is in the bright state (since the mode $f_k$ is then occupied). We will assume that this phase shift can be corrected experimentally. For simplicity we examine the situation, where for all arms, we obtain the measurements $t_k = 1$ and $b_k = 0$. The measurement described by Eq. \ref{NoErrors:Equation:ParticularMeasurement} then transforms the state as:
\begin{align}
	\ket{\psi} \ket{L} \rightarrow \left(\frac{1}{\sqrt{2}}\right)^N \prod_{k=1}^{N} (\bra{0}_{f_k}\bra{1}_{l_k} + \bra{1}_{f_k}\bra{0}_{l_k})  \ket{\psi} \ket{L}
	\label{Analysis:equation:projection}
\end{align}
Note that we haven't renormalized, and the norm of the state has been reduced.\\
Evidently, if mode $l_k$ contains 1 photon, then mode $f_k$ is vacant, and the qubit state must be $\ket{0}_{q_k}$ (dark). Vice versa if mode $l_k$ contains no photons.
We rewrite the projective measurement as:
\begin{align}
\prod_{k=1}^{N} (\bra{0}_{f_k}\bra{1}_{l_k} + \bra{1}_{f_k}\bra{0}_{l_k}) = \sum_{\mathbf{m}} \bra{\lnot\mathbf{m}}_f \bra{\mathbf{m}}_l
\label{NoErrors:Equation:Measurement}
\end{align}
Where $\mathbf{m}$ is any binary list of length $N$. $\lnot\mathbf{m}$ should be understood as the negation (not) of $\mathbf{m}$. 
Using Eq. \ref{NoErrors:Equation:psi1}, \ref{NoErrors:Equation:Register}, \ref{Analysis:equation:projection}, and \ref{NoErrors:Equation:Measurement}, the result of the measurement is:
\begin{align}
	\ket{\psi} \ket{L} \rightarrow \ket{\alpha} =  \left(\frac{1}{\sqrt{2}}\right)^N \sum_{n=0}^{\infty} \sum_{\mathbf{j}_n}   \sum_{\mathbf{a}} \sum_{\mathbf{m}} c_n \frac{1}{\sqrt{n!}} \left( \frac{1}{\sqrt{N}} \right)^n \beta(\mathbf{a},\theta_L) \Omega_{\mathbf{j}_n} \bra{\lnot\mathbf{m}}_f \ket{\mathbf{a}}_f \ket{\mathbf{a}}_q \bra{\mathbf{m}}_l\ket{\mathbf{j}_n}_l  \ket{n}_R 
\end{align}
Since $\mathbf{m}$ is a binary list, then the overlap $\bra{\mathbf{m}}_l \ket{\mathbf{j}_n}_l$ is only non-zero when  the optical input from the TMSV state $\mathbf{j}_n$ is also binary. This implies:
\begin{align}
	\Omega_{\mathbf{j}_n} = n!
\end{align}
Conditioned on the overlap $\bra{\mathbf{m}}_l \ket{\mathbf{j}_n}_l$ being non-zero, we see that $\mathbf{a}$ must be the negation of $\mathbf{j}_n$ so that $\bra{\lnot\mathbf{m}}_f\ket{\mathbf{a}}_f$ is also non-zero. This implies that the state shared between the right TMSV and the left registry after measurement is:
\begin{align}
	\ket{\alpha} =\left(\frac{1}{\sqrt{2}}\right)^N \sum_{n=0}^{N} \sum_{\mathbf{j}_n} c_n \left( \frac{1}{\sqrt{N}} \right)^n \beta(n,\theta_L)  \sqrt{n!} \ket{\lnot \mathbf{j}_n}_{L}  \ket{n}_R 
\end{align}
Where $\ket{\lnot \mathbf{j}_n}_{L}$ is the state of the qubits in the left register. We've neglected the subscript $q$ since there can no longer be any confusion as to what subsystem the vector describes. The sum over $n$ has been terminated at $N$, since no binary string $\mathbf{j}_n$ exist for $n>N$. We've also used the fact that:
\begin{align}
    \beta(\mathbf{a},\theta_L) = \beta(\lnot \mathbf{j}_n,\theta_L) = \beta(n,\theta_L) = \cos(\theta_L)^{n} \sin(\theta_L)^{N-n}
\end{align}
We may perform the sum over $\mathbf{j}_n$, introducing the vector:
\begin{align}
    \sum_{\mathbf{j}_n} \ket{\lnot \mathbf{j}_n}_{L} = \binom{N}{n}^{1/2} \ket{\mathbf{I}_{N-n}}_L
\end{align}
Where $\ket{\mathbf{I}_{N-n}}_L$ is normalized and is an even superposition of all binary states containing $N-n$ bright state qubits and $n$ dark state qubits.
Comparing with the original TMSV state, we see that the left register transforms a Fock state as:
\begin{align}
    \ket{n} &\rightarrow \left(\frac{1}{\sqrt{2}}\right)^N \left( \frac{1}{\sqrt{N}} \right)^n \beta(n,\theta_L)  \sqrt{n!} \binom{N}{n}^{1/2} \ket{\mathbf{I}_{N-n}} \\ &=  \Delta(n,\theta_L)  \ket{\mathbf{I}_{N-n}}
    \label{NoError:Equation:FockTransform}
\end{align}
Where
\begin{align}
	\Delta(n,\theta_L) = \left(\frac{1}{\sqrt{2}}\right)^N \binom{N}{n}^{1/2} \left( \frac{1}{\sqrt{N}} \right)^n    \sqrt{n!} \beta(n,\theta_L)
\end{align}
Using this transform, and assuming no loss in the fiber, we may infer that storing the right part of the TMSV in the right register (see Fig. \ref{Analysis:Figure:Layout}), results in the state:
\begin{align}
	\ket{\alpha} = \sum_{n=0}^{N} c_n  \Delta(n,\theta_L) \Delta(n,\theta_R)  \ket{\mathbf{I}_{N-n}}_L \ket{\mathbf{I}_{N-n}}_R
	\label{NoErrors:Equation:Final1}
\end{align}
We may then compute the norm of the state of the two registries:
\begin{align}
    \braket{\alpha|\alpha} &= \sum_{m=0}^{N} |c_m|^2 |\Delta(m,\theta_L)|^2 |\Delta(m,\theta_R)|^2 
\end{align}
The probability of successful entanglement sharing between the 2 registries is then this norm multiplied by the number of measurements that would yield an equivalent state. For each arm we have 2 detector outcomes, (0,1) or (1,0), that would yield a state equivalent to the one described above. The probability of successful entanglement sharing is then:
\begin{align}
    P_s = 2^N 2^N \braket{\alpha|\alpha} = 4^N \braket{\alpha|\alpha}
\end{align}

\subsubsection{Performance with Loss}
We initialize the optical channel in a TMSV state:
\begin{equation}
	\ket{\psi} = \sum_{n=0}^{\infty} c_n \ket{n}_L\ket{n}_R
\end{equation}
We send the right part of the TMSV through a lossy channel modelled by a beamsplitter with transmission amplitude $\sqrt{\eta_R}$. The transmittance of the fiber is then given by $\eta_R$. Likewise we send the left part of the TMSV state through a lossy channel of transmittance $\eta_L$  The channels transforms the state as:
\begin{equation}
	\ket{\psi} \rightarrow \sum_{n=0}^{\infty} \sum_{l_R=0}^{n} \sum_{l_L=0}^{n} \epsilon_R(n,l_R) \epsilon_L(n,l_L)  c_n \ket{n-l_L}_L \ket{n-l_R}_R \ket{l_L}_{e_L} \ket{l_R}_{e_R} 
\end{equation}
Where $e_R$ is a loss channel. The loss amplitude is given as:
\begin{equation}
	\epsilon_{R/L}(n,l_{R/L}) = \sqrt{\binom{n}{n-l_{R/L}}} \eta_{R/L}^{(n-l_{R/L})/2} (1-\eta_{R/L})^{l_{R/L}/2}
\end{equation}
Inserting the Fock state transform Eq. \ref{NoError:Equation:FockTransform}, we arrive at the register state:
\begin{align}
	\ket{\alpha} = \sum_{n=0}^{N} \sum_{l_L=0}^{n} \sum_{l_R=0}^{n} c_n \epsilon_L(n,l_L) \epsilon_R(n,l_R) \Delta(n-l_L,\theta_L) \Delta(n-l_R,\theta_R) \ket{\mathbf{I}_{N-n+l_L}}_L   \ket{\mathbf{I}_{N-n+l_R}}_R \ket{l_L}_{e_L}  \ket{l_R}_{e_R} 
	\label{NoError:Equation:Lossy}
\end{align}
The corresponding density matrix is:
\begin{align}
	\sigma &= \sum_{n=0}^{N} \sum_{m=0}^{N} \sum_{l_L=0}^{n} \sum_{k_L=0}^{m} \sum_{l_R=0}^{n} \sum_{k_R=0}^{m} c_n c_m^* \epsilon_R(n,l_R) \epsilon_L(n,l_L) \epsilon_R(m,k_R)^* \epsilon_L(m,k_L)^*  \nonumber \\& \Delta(n-l_L,\theta_L) \Delta(n-l_R,\theta_R) \Delta(m-k_L,\theta_L)^* \Delta(m-k_R,\theta_R)^* \nonumber \\&  \ket{\mathbf{I}_{N-n+l_L}}_L \bra{\mathbf{I}_{N-m+k_L}}_L   \ket{\mathbf{I}_{N-n+l_R}}_R \bra{\mathbf{I}_{N-m+k_R}}_R \ket{l_L}_{e_L} \bra{k_L}_{e_L} \ket{l_R}_{e_R} \bra{k_R}_{e_R}
\end{align}
We then trace out the loss channel, giving the state:
\begin{align}
	\rho &= \text{Tr}_e \sigma = \sum_{n=0}^{N} \sum_{m=0}^{N} 
	\sum_{l=0}^{\texttt{min}(n,m)} 
	\sum_{r=0}^{\texttt{min}(n,m)} 
	c_n c_m^* \epsilon_R(n,r) \epsilon_L(n,l) \epsilon_R(m,r)^* \epsilon_L(m,l)^*  \nonumber \\& \Delta(n-l,\theta_L) \Delta(n-r,\theta_R) \Delta(m-l,\theta_L)^* \Delta(m-r,\theta_R)^* \nonumber \\&  \ket{\mathbf{I}_{N-n+l}}_L \bra{\mathbf{I}_{N-m+l}}_L   \ket{\mathbf{I}_{N-n+r}}_R \bra{\mathbf{I}_{N-m+r}}_R 
\end{align}
We define the matrix elements:
\begin{align}
    \Lambda(n,m,l,r) &= c_n c_m^* \epsilon_R(n,r) \epsilon_L(n,l) \epsilon_R(m,r)^* \epsilon_L(m,l)^*  \nonumber \\& \Delta(n-l,\theta_L) \Delta(n-r,\theta_R) \Delta(m-l,\theta_L)^* \Delta(m-r,\theta_R)^*
	\label{Analysis:Registers:Equation:Lambda}
\end{align}
Such that we may write the state as:
\begin{align}
    \rho = \sum_{n=0}^{N} \sum_{m=0}^{N} \sum_{l=0}^{\texttt{min}(n,m)} \sum_{r=0}^{\texttt{min}(n,m)} \Lambda(n,m,l,r) \ket{\mathbf{I}_{N-n+l}}_L \bra{\mathbf{I}_{N-m+l}}_L   \ket{\mathbf{I}_{N-n+r}}_R \bra{\mathbf{I}_{N-m+r}}_R
    \label{NoError:Equation:TracedDensityLoss}
\end{align}

\subsubsection{One Qubit Per Register}
\label{Analysis:SingleQubitCase}
In the following we will analyse the case of one sided loss. Loss is assumed to only occur between the EPR source and the right register in each repeater. If $N=1$ then we have the density matrix:
\begin{align}
    &\rho = \nonumber \\&\frac{1}{4} \begin{pmatrix}
    |c_1|^2 \eta \cos(\theta_L)^{2}  \cos(\theta_R)^{2} & 0 & 0 &  c_1 c_0^* \sqrt{\eta} \sin(\theta_R) \sin(\theta_L) \cos(\theta_R) \cos(\theta_L) \\
    0 & |c_1|^2 (1-\eta) \cos(\theta_L)^2 \sin(\theta_R)^2 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    c_1^* c_0 \sqrt{\eta} \sin(\theta_R) \sin(\theta_L) \cos(\theta_R) \cos(\theta_L) & 0 & 0 & |c_0|^2 \sin(\theta_L)^2 \sin(\theta_R)^2 \\
    \end{pmatrix}
    \label{Analysis:Equation:1QubitLossy}
\end{align}

If we use the above state for entanglement swapping via Bell measurements, there is an advantage in keeping the matrix elements $\rho_{11}$ and $\rho_{44}$ identical. If this is not the case, series of swaps will tend to make the state more separable and thereby diminish entanglement.
%This can be seen in the pure state case, let the state of the two pairs of registers be:
%\begin{align}
%    \ket{\Psi} &= \ket{\psi_1} \otimes \ket{\psi_2}
%\end{align}
%With
%\begin{align}
%    \ket{\psi_1} &= b_1 \ket{0}_{L_1}\ket{0}_{R_1} + b_0 \ket{1}_{L_1}\ket{1}_{R_1} \\
%    \ket{\psi_2} &= b_1 \ket{0}_{L_2}\ket{0}_{R_2} + b_0 \ket{1}_{L_2}\ket{1}_{R_2} \\
%\end{align}
%We then perform a Bell measurement by projecting onto:
%\begin{equation}
%    \ket{\psi_{-}} = \frac{1}{\sqrt{2}} \left( \ket{0}_{R_1}\ket{0}_{L_2} - \ket{1}_{R_1}\ket{1}_{L_2} \right)
%\end{equation}
%Giving:
%\begin{equation}
%    \ket{\Psi} \rightarrow \frac{1}{\sqrt{2}} \left( b_1^2 \ket{0}_{L_1} \ket{0}_{R_2} - b_0^2 \ket{1}_{L_1} \ket{1}_{R_2}   \right)
%\end{equation}
%Clearly if $|b_0|>|b_1|$ then $|b_0^2|\gg|b_1|^2$, or vice versa, and the state becomes increasingly separable as we perform many swaps, greatly diminishing the entanglement between Alice and Bob. Only if the amplitudes are equal or almost equal does the state serve as a good resource for swapping using Bell measurement. In general we find that the state which is ideal for entanglement swapping, is also maximally entangled. With 1 qubit per register we want $\rho_{11} = \rho_{44}$, or:\\
This constraint implies:
\begin{align}
        |c_1|^2 \eta \cos(\theta_L)^{2}  \cos(\theta_R)^{2} = |c_0|^2 \sin(\theta_L)^2 \sin(\theta_R)^2
\end{align}
This implies a bond between $\theta_R$ and $\theta_L$.
\begin{align}
    \tan(\theta_L)^2 = \tan(\theta_R)^{-2} \eta \frac{|c_1|^2}{|c_0|^2}
    \label{Analysis:Equation:Bond}
\end{align}
Utilizing the bond in Eq. \ref{Analysis:Equation:Bond} we may rewrite the density matrix as:
\begin{align}
    \rho = \frac{1}{4} \frac{\sin(\theta_R)^2 |c_1|^2 |c_0|^2 \eta}{ \tan(\theta_R)^2 |c_0|^2+ \eta |c_1|^2} \begin{pmatrix}
    1   & 0 & 0 &  -e^{i \phi} \\
    0 &  (\eta^{-1}-1)  \tan(\theta_R)^2 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    -e^{-i \phi}    & 0 & 0 & 1 \\
    \end{pmatrix}
    \label{Analysis:Equation:1QubitLossy-2}
\end{align}
We now want to choose the superposition angle $\theta_R$ that maximizes the signal-to-noise ratio of measurements performed at the two registers. We will consider measurements performed in bright/dark (1,0) basis. In this work the state is transmitted through a lossy fiber, for which the only source of noise is the loss of photons to the environment. For this reason we consider the signal-to-noise ratio given by:
\begin{align}
     \mathcal{S}/\mathcal{N} = \frac{\rho_{11} + \rho_{44}}{\rho_{22}}
\end{align}
Where $\rho_{ij}$ are elements of the density matrix. The probabilities $\rho_{11}$ and and $\rho_{44}$, correspond to correlated measurement outcomes at the two registers, whereas the loss term, $\rho_{22}$, correspond to uncorrelated outcomes. This motivates the above quantity as a measure of the signal-to-noise ratio. We may rewrite $\mathcal{S}/\mathcal{N}$ as:
\begin{align}
     \mathcal{S}/\mathcal{N} = \frac{\Lambda(1,1,0) + \Lambda(0,0,0)}{\Lambda(1,1,1)} = \frac{2}{(\eta^{-1}-1)  \tan(\theta_R)^2}
\end{align}
Which we maximize when $\theta_R \rightarrow 0$. Evidently, we may suppress the noise term $\rho_{22}$, corresponding to information lost to Eve, by letting $\theta_R$ tend to zero.\\ 
However, there is one more condition to consider. The probability of the measurements at the photodetectors succeeding, which goes to zero in this limit where $\theta_R \rightarrow 0$.
The probability of success is given by the trace of $\rho$:
\begin{align}
    P(\theta_R,\langle n \rangle;\eta) = \sin(\theta_R)^2 |c_1|^2 |c_0|^2 \frac{ 2 \eta + (1-\eta)  \tan(\theta_R)^2}{ \tan(\theta_R)^2 |c_0|^2+ \eta |c_1|^2}
    \label{Analysis:Equation:ProbabilityThetaR}
\end{align}
Where we take into account that the measurements at the photodetectors can succeed in 4 ways. The optimal choice of $\theta_R$ is then the choice that maximizes $\mathcal{S}/\mathcal{N}$ subject to the condition that:
\begin{align}
    P(\theta_R,\langle n \rangle;\eta) \geq \epsilon
    \label{Analysis:Equation:Epsilon}
\end{align}
Where $\epsilon$ is  the minimum probability of success tolerated by the experimental setup. 
We may optimize $P(\theta_R,\langle n \rangle;\eta)$ in $\langle n \rangle$ for a given $\theta_R$ and $\eta$ by squeezing the TMSV source such that we have the equality:
\begin{align}
    \langle n \rangle = \sqrt{1-\frac{\eta}{\eta + \tan\left(\theta_R \right)^2}}
\end{align}
%Using this we may refine the requirement on $\theta_R$: We should choose $\theta_R$ such that we maximize $\mathcal{S}/\mathcal{N}$ while obeying the constraint:
%\begin{align}
%    \text{max} \{ P(\theta_R,\langle n \rangle;\eta) \}_{\langle n \rangle} \geq %\epsilon
%    \label{Analysis:Equation:Epsilon}
%\end{align}
%The brackets indicating that we have set $\langle n \rangle$ to the value that %maximizes the probability. \\
Inserting the optimal choice of $\langle n \rangle$ into $P(\theta_R,\langle n \rangle;\eta)$ we obtain the probability  $P(\theta_R;\eta)$. From numerical investigation we find that this probability depends on the angle $\theta_R$ in a complicated manner. However, for values of $\theta_R$ below $\sim 0.66$ we have that the probability decreases monotonically in $\theta_R$ for any value of $\eta$. In order to increase the signal-to-noise ratio of the transmitted signal we require low values of $\theta_R$, and so we expect to be below this angle. With this consideration, we may assume that the signal-to-noise ratio is optimized when:
\begin{align}
    P(\theta_R;\eta) = \epsilon
    \label{Analysis:Equation:thetaR}
\end{align}
Which can be rewritten as a quartic polynomial equation in $z=\sqrt{1-\frac{\eta}{\eta+\tan(\theta_R)^2}}$:
\begin{align}
    \epsilon + 2 \epsilon z + \eta \left[ \epsilon -2 \right] z^2 + \epsilon \left[ 2 \eta - 2 \right] z^3 + \left[ -\epsilon + (1+\epsilon) \eta + \eta^2 \right] z^4 = 0
\end{align}
Which can be solved efficiently numerically and from which we can find $\theta_R$.\\

Given that we've made the optimal choice of $\theta_R$ we can investigate how the state evolves under a sequence of swaps. Obtaining the particular Bell measurement outcome corresponding to the ket $\ket{\psi} = \frac{1}{\sqrt{2}} \left( \ket{0_{R_1}0_{L_2}} + \ket{1_{R_1}1_{L_2}} \right)$ on registers $R_1$ and $L_2$, we obtain the state:
\begin{align}
    \rho_f = \frac{1}{2} (\bra{0_{R_1}0_{L_2}} + \bra{1_{R_1}1_{L_2}}) \Omega (\ket{0_{R_1}0_{L_2}} + \ket{1_{R_1}1_{L_2}})
\end{align}
With $\Omega$ given by Eq. \ref{Analysis:Equation:ProdState}. We may evaluate $\rho_f$ by using the state given in Eq. \ref{Analysis:Equation:1QubitLossy-2}. We obtain the unormalized state:
\begin{align}
    \rho_f = \frac{1}{2} \left( \frac{1}{4} \frac{\sin(\theta_R)^2 |c_1|^2 |c_0|^2 \eta}{ \tan(\theta_R)^2 |c_0|^2+ \eta |c_1|^2} \right)^2 \begin{pmatrix}
    1   & 0 & 0 &  \left(-e^{i \phi}\right)^2 \\
    0 &  2 (\eta^{-1}-1)  \tan(\theta_R)^2 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    \left(-e^{-i \phi} \right)^2    & 0 & 0 & 1 \\
    \end{pmatrix}
\end{align}
Clearly the state is similar in structure to the original state, with the loss term having doubled in size. Continuing this, then after $s$ swaps we obtain the unnormalized density matrix: 
\begin{align}
    \rho_f = \left(\frac{1}{2} \right)^s \left( \frac{1}{4} \frac{\sin(\theta_R)^2 |c_1|^2 |c_0|^2 \eta}{ \tan(\theta_R)^2 |c_0|^2+ \eta |c_1|^2} \right)^{s+1} \begin{pmatrix}
    1   & 0 & 0 &  \left(-e^{i \phi}\right)^{s+1} \\
    0 &  (s+1) (\eta^{-1}-1)  \tan(\theta_R)^2 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    \left(-e^{-i \phi} \right)^{s+1}    & 0 & 0 & 1 \\
    \end{pmatrix}
\end{align}
Of course, other Bell measurements than the one considered here will occur. We will numerically simulate swaps by randomly drawing from the four Bell measurements using a Metropolis-Hastings algorithm as will be outlined in section \ref{MetropolisHastings:Section}.

%\subsubsection{N Qubits per Register}
%With N qubits per register we have the state
%\begin{align}
%    \rho &=  \sum_{n=0}^{N} \sum_{m=0}^{N} \sum_{l=0}^{\texttt{min}(n,m)} \Lambda(n,m,l) \ket{\mathbf{I}_{N-n}}_{L} \bra{\mathbf{I}_{N-m}}_{L}   \ket{\mathbf{I}_{N-n+l}}_{R} \bra{\mathbf{I}_{N-m+l}}_{R}
%    \label{Analysis:Equation:2qubitState}
%\end{align}
%We can derive the signal-to-noise ratio from the probabilities given by Eq. %\ref{Analysis:Registers:Equation:Lambda}. The result is given by:
%\begin{align}
%    \mathcal{S}/\mathcal{N} &= \frac{\Lambda(0,0,0)+\Lambda(1,1,0)+\Lambda(2,2,0)}{\Lambda(1,1,1)+\Lambda(2,2,1)+\Lambda(2,2,2)} \\
    %&= \frac{|c_0|^2 \sin(\theta_L)^4 \sin(\theta_R)^4 + |c_1|^2 \eta \sin(\theta_L)^2 \cos(\theta_L)^2 \sin(\theta_R)^2 \cos(\theta_R)^2 + |c_2|^2 (\eta^2/4) \cos(\theta_L)^4 \cos(\theta_R)^4 }{|c_1|^2(1-\eta) \sin(\theta_L)^2 \cos(\theta_L)^2 \sin(\theta_R)^4 + |c_2|^2 \eta (1-\eta) \cos(\theta_L)^4 \sin(\theta_R)^2 \cos(\theta_R)^2 + |c_2|^2 \left((1-\eta)^2/2\right) \cos(\theta_L)^4 \sin(\theta_R)^4}\\
    %&= \frac{|c_0|^2 \sin(\theta_L)^4 + |c_1|^2 \eta \sin(\theta_L)^2 \cos(\theta_L)^2 \tan(\theta_R)^{-2} + |c_2|^2 (\eta^2/4) \cos(\theta_L)^4 \tan(\theta_R)^{-4} }{|c_1|^2(1-\eta) \sin(\theta_L)^2 \cos(\theta_L)^2 + |c_2|^2 \eta (1-\eta) \cos(\theta_L)^4 \tan(\theta_R)^{-2} + |c_2|^2 \left((1-\eta)^2/2\right) \cos(\theta_L)^4}\\
    %&= \frac{|c_0|^2 \tan(\theta_L)^4 + |c_1|^2 \eta \tan(\theta_L)^2 \tan(\theta_R)^{-2} + |c_2|^2 (\eta^2/4) \tan(\theta_R)^{-4} }{|c_1|^2(1-\eta) \tan(\theta_L)^2 + |c_2|^2 \eta (1-\eta) \tan(\theta_R)^{-2} + |c_2|^2 \left((1-\eta)^2/2\right)}\\
%    &= \frac{|c_0|^2 \tan(\theta_L)^4 \tan(\theta_R)^4 + |c_1|^2 \eta \tan(\theta_L)^2 \tan(\theta_R)^{2} + |c_2|^2 (\eta^2/4)}{|c_1|^2(1-\eta) \tan(\theta_L)^2 \tan(\theta_R)^4 + |c_2|^2 \eta (1-\eta) \tan(\theta_R)^{2} + |c_2|^2 \left((1-\eta)^2/2\right) \tan(\theta_R)^4}
%\end{align}
%Which is maximized when $\theta_R$ tends to zero. Evidently we wish to make %$\theta_R$ as small as possible subject to some lowest accepted probability of %success.\\
%Unfortunately the state given in Eq. \ref{Analysis:Equation:2qubitState} will not serve as a good resource for teleportation, since we cannot make $\Lambda(n,n,0)$ equal for all $n$ with any choice of $\theta_L$, $\theta_R$, and $\langle n \rangle$. Subsequent swaps will tend to make the state separable as discussed in the previous section. 

%This problem can be overcome by acting with a filter on the right register which makes the signals equal. This filter is in the form of a POVM given by the set of projectors:
%\begin{align}
%    \Pi_1^{(N)} &= \text{min} \{ \sqrt{\Lambda(i,i,0)} \}_i \sum_{j=0}^N \frac{1}{\sqrt{\Lambda(j,j,0)}} \ket{I_{N-j}}_{R} \bra{I_{N-j}}_{R} \\
%    \Pi_2^{(N)} &= I - \Pi_1^{(N)}
%\end{align}
%Where $\text{min} \{ \sqrt{\Lambda(i,i,0)} \}_i$ is the smallest amplitude in the set $\{ \sqrt{\Lambda(i,i,0)} \}_i$ generated by $i \in [0,N]$. 
%Acting with this filter we obtain the unormalized state:
%\begin{align}
%    \rho =  \text{min} \{ \Lambda(i,i,0) \}_i \sum_{n=0}^{N} \sum_{m=0}^{N} \sum_{l=0}^{\texttt{min}(n,m)} & \frac{\Lambda(n,m,l)}{\sqrt{\Lambda(n-l,n-l,0) \Lambda(m-l,m-l,0) }} \nonumber \\ &\ket{\mathbf{I}_{N-n}}_{L} \bra{\mathbf{I}_{N-m}}_{L}   \ket{\mathbf{I}_{N-n+l}}_{R} \bra{\mathbf{I}_{N-m+l}}_{R}
%    \label{Analysis:Equation:2qubitStateFiltered}
%\end{align}
%For which $\Lambda(n,n,0)$ are equal for all $n$. We then choose $\theta_L$, $\theta_R$, and $\langle n \rangle$ such that the secret key of this bipartite state is maximal. The computation of the secret key is outlined in section \ref{Section:SecretKey}. We maximize the secret key in $\theta_L$, $\theta_R$, and $\langle n \rangle$ numerically using the SciPy implementation of the Nelder-Mead algorithm \cite{han12}. The optimization is constrained by the requirement that the probability of successful entanglement sharing must be larger than some lowest acceptable value $\epsilon$:
%\begin{align}
%    P(\theta_R,\theta_L,\langle n \rangle;\eta) \geq \epsilon
%\end{align}


%The signal-to-noise ratio is now:
%\begin{align}
%    \mathcal{S}/\mathcal{N} &= \frac{N+1}{\sum^N_{n=0} \sum^n_{l=1} \Lambda(n,n,l) \left[ \Lambda(n-l,n-l,0) \right]^{-1}} \\ 
%    &= \frac{N+1}{\sum^N_{n=0} \sum^n_{l=1} f(n,l) \left[ \tan(\theta_L) \tan(\theta_R) \right]^{-2l}}
%\end{align}
%With
%\begin{align}
%    f(n,l) = 
%\end{align}
%Let
%\begin{align}
%    P(\theta_R,\theta_L,\langle n \rangle; \eta) = p
%\end{align}
%Then
%\begin{align}
%    p = \text{min} \{ \Lambda(i,i,0) \}_i \left[ N + 1 + \sum^N_{n=0} \sum^n_{l=1} f(n,l) \left[ \tan(\theta_L) \tan(\theta_R) \right]^{-2l} \right]
%\end{align}





==> Text/Results.tex <==
\section{Results}
In this section we show the results of this work based on the mathematical analysis presented in the previous section. We will be using the negativity to characterize the entanglement between registers, and the secret key rate to gauge the possibility of transmitting a secret key.\\






%\subsubsection{Two Qubit Registers}
%We now investigate the case of two qubits per register. The secret key rate can be seen in Fig. \ref{Results:Figure:SKsvsDistN2}. The values of $\theta_R$, $\theta_L$, and $\langle n \rangle$ are found from a numerical optimization of the secret key between pairs of registers. One can argue that it would be better to optimize the secret key rate for the whole repeater array. However, we find that the secret key rate is a stochastic parameter, slightly dependent on what Bell measurements are realized during swaps. This randomness makes it difficult to directly optimize the secret key rate. When comparing the plot in Fig. \ref{Results:Figure:SKsvsDistN2} with the plot in Fig. \ref{Results:Figure:SKsvsDist} it is quite clear that the repeater scheme fares much worse with two qubits. Clearly we require far more attempts before we can generate a secret key at large distances. This is mainly because it is more improbable to generate the register state. In order to generate a very pure state (low $\theta_R$) we must then use many more attempts than for the 1 qubit case. This impacts the rate, and we observe that we beat the PLOB bound at significantly larger distances. The wiggles in the secret key rate are suspected to be caused by the optimization routine and its stochastic properties.
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{Figures/SKvsDistN2s.png}
%\caption{\textit{Plot of the secret key rate obtained with 2 qubit per register against the distance between sender and receiver. The allowed number of attempts $A$ is shown in the legend. The register separation distance is 7 km which was found to be optimal. Each plot is an average of 25 calculations.}}
%\label{Results:Figure:SKsvsDistN2}
%\end{figure}




\newpage



%We then turn to numerical simulations to investigate how entanglement swapping based on single qubit registries can be used to share entanglement between distant nodes, and whether the considered setup can beat the PLOB bound under realistic conditions, that is we consider the photodetectors to be photon resolving as well as click detectors. We model the channel as a lossy channel using the Krauss operator:
%\begin{align}
%    E_l = \left( \frac{\gamma}{1-\gamma}\right)^{l/2} \frac{\hat{a}^l}{\sqrt{l!}} \left(1-\gamma\right)^{\hat{n}/2}
%\end{align}
%With the corresponding mapping of the state being:
%\begin{align}
    %\rho \rightarrow \sum_{l=0}^{\infty} E_l \rho E_l^{\dagger}
%\end{align}
%The channel consists of many pairs of registers which we desire to entangle using the proposed scheme. When all the pairs of registers are entangled we may generate entanglement between distant nodes by swapping. However, the probability of all entangling measurements succeeding at first attempt rapidly decreases. For this reason we must gauge how many attempts are necessary before all pairs of registers are entangled. This number of attempts should be used to normalize the secret key in order to obtain the secret key rate. The average number of attempts needed before all entangled links are formed, and swapping can be begin, is given from the expression:
%\begin{align}
%    Z_n(P) = \sum_{j=1}^{2^n} \binom{n}{j} \frac{\left(-1\right)^{j+1}}{1-(1-P)^j}
%\end{align}
%Where $n$ is the number of entangled links we need to form. \\
%Initially we consider the case where the photodetectors are perfectly photon resolving and have unit collection efficiency. In this case, we can compute the secret key rate and plot it. This is shown in Fig. \ref{Results:Figure:PhotonResolving}. We observe that we can beat the PLOB bound at a total distance of about 225 km. The link distance is set at 10 km.\\
%\begin{figure}[h]
%\centering
%\includegraphics[width=1\textwidth]{Figures/CL0.05-Eta0.95-v0-l10.png}
%\caption{\textit{asd}}
%\label{Results:Figure:PhotonResolving}
%\end{figure}
%We then turn to the more realistic scenario where the photodetectors are click detectors, modelled by the projective map:
%\begin{align}
    %\Pi_{off} = e^{-\nu} \sum_{n=0}^{\infty} \left( 1 - \eta_{PD} \right)^{n} \ket{n} \bra{n}
%\end{align}
%Where $\nu$ is the rate of dark counts and $\eta_{PD}$ is the collection efficiency of the photodetector. We set the dark count rate at 0, but we will shortly consider what happens when it is non-zero. \\

%The secret key rate against total distance for a link distance of 10 km is shown in Fig. \ref{Results:Figure:ImperfectDetectorSK}. We observe that the repeater beats the PLOB bound if the collection efficiency is above 75 \%. For instance, if the collection efficiency is 95 \% then the repeater beats the PLOB bound at around 300 km. However, there is a cost to pay. At this distance, we require 30 entangled links, and the number of attempts before entanglement is established grows to large numbers. This number of attempts is plotted in Fig. \ref{Results:Figure:ImperfectDetectorTrials}. The figure shows that if the collection efficiency is 95 \%, then we require in the vicinity of $10^{5}$ attempts before entanglement can be established, if however a single dark count happens during these attempts, then the protocol fails.
%\begin{figure}[h]
%\centering
%\includegraphics[width=1\textwidth]{Figures/imperfectDetectorKs.png}
%\caption{\textit{asd}}
%\label{Results:Figure:ImperfectDetectorSK}
%\end{figure}

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\textwidth]{Figures/imperfectDetectorTrials.png}
%\caption{\textit{asd}}
%\label{Results:Figure:ImperfectDetectorTrials}
%\end{figure}
